Fundamental Limits of Transferability and Equivariance in Algebraic Signal Models I: Finite Dimensions

We study the fundamental limits of transferability in algebraic signal processing through homomorphisms between algebraic signal models. Homomorphisms are linear maps between the signal spaces of two models that commute with filtering, so filtering a signal and transferring it across domains can be done in either order. The existence of such maps is governed entirely by coincidences among the filtered eigenvalues of the two models' shift operators, but existence alone is insufficient: the space of homomorphisms always contains trivial elements that destroy all information. We introduce the spectral transfer efficiency $\eta(\theta)\in[0,1]$ to quantify information-preserving quality, prove that every homomorphism decomposes into unconstrained blocks over coincidence classes, derive the dimension of the homomorphism space, and characterize exactly when lossless transfer is achievable. Beyond normal shift operators, we quantify a departure-from-normality penalty and show how filter derivatives can repair spectral defectiveness. The theory yields concrete consequences in three settings: for sampling, eigenvalue interlacing converts transferability under subsampling into an explicit filter design constraint; for compressed sensing, $\eta(\theta)$ controls the restricted isometry constant and the coherence of the resulting measurements, and recovery decouples across coincidence classes; and for machine learning, spectral aliasing emerges as the controlled symmetry breaking that makes transfer between mismatched domains possible at all.

==> latex_resources/mySections.tex <==
\usepackage{needspace}

% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\bf #1}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\medskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}



==> source_figs/fig1/fig1_tikz_source.tex <==
%!TEX root = fig1_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%%-------Blue Colors of the Palette
\definecolor{my_alejocol5a}{RGB}{1,31,75}
\definecolor{my_alejocol4a}{RGB}{3,57,108}
\definecolor{my_alejocol3a}{RGB}{0,91,150}
\definecolor{my_alejocol2a}{RGB}{100,151,177}
\definecolor{my_alejocol1a}{RGB}{179,205,224}

%--------Red Colors of the Palette
\definecolor{my_alejocol4b}{RGB}{212, 220, 220}
\definecolor{my_alejocol3b}{RGB}{113, 18, 55}
\definecolor{my_alejocol2b}{RGB}{236, 85, 141}
\definecolor{my_alejocol1b}{RGB}{225, 73, 132}

%--------Blue-Green Colors of the Palette
\definecolor{my_alejocol4c}{RGB}{81, 185, 239}
\definecolor{my_alejocol3c}{RGB}{119, 164, 211}
\definecolor{my_alejocol2c}{RGB}{193, 223, 213}
\definecolor{my_alejocol1c}{RGB}{53, 89, 85}

%--Gray colors added to the pallette
\colorlet{my_alejocolg1}{black!30}
\colorlet{my_alejocolg2}{black!35}
\colorlet{my_alejocolg3}{black!40}
\colorlet{my_alejocolg4}{black!45}
\colorlet{my_alejocolg5}{black!50}
\colorlet{my_alejocolg6}{black!55}
\colorlet{my_alejocolg7}{black!60}



\usetikzlibrary{positioning,decorations.pathreplacing,shapes}
%\usepackage[english]{babel}
%\usepackage{microtype}
%\usepackage[hmargin=1.5cm,vmargin=1cm]{geometry}
%\usepackage{amsmath}
%\DeclareMathOperator{\p}{p}
%\newcommand*{\cancer}{\text{cancer}}
%\newcommand*{\testp}{\text{test}+}



%%%%%%%%%%%%%%%%%%%%%%%%%%% Settings of Blocks and picture %%%%%%%%%%%%%%%%%%%

\def \scale {1.3}
\def \unit  { \scale cm}
\def \layerinterdist {2.5}


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0.2*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]

                    
\tikzstyle{vectorspace} = [ set, 
                             fill=my_alejocol4c!50,
                             minimum width  = 1.5*\unit,
                             minimum height = 2.0*\unit]
                             
\tikzstyle{endomorphisms} = [ vectorspace,
                              fill=black!15,
                              minimum height = 1.3*\unit]
                                
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in1} = [endomorphisms, rounded corners=0.3*\unit,
                              fill=black!30,
                              minimum width  = 0.8*\unit,
                              minimum height = 0.8*\unit
                             ]                                                                                                                                                
\tikzstyle{algebra} = [ endomorphisms,
                        fill=my_alejocol2b!70,
                        minimum width = 1.5*\unit]


\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





{\fontsize{8}{8}\selectfont


\begin{tikzpicture}[rounded corners,ultra thick]




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Vector space M  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (0,0) node [vectorspace] (M0) {};
   \path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};
   
   % Element of the vector space
   \path (M0) ++ (-0.5,0.2) node [dot] (x) {};
   \path (x.south)++(0,-0.1) node [below, color=black] {$\mathbf{x}$}; 
   
   % Element filtered in the vector space
   \path (M0) ++ (0.5,0.2) node [dot] (ex) {};
   \path (ex.south) node [below, color=black] {$\rho(a)\mathbf{x}$};      
              

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Endomorphisms   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   % Space of endomorphisms
   \path (M0.north) ++ (0, 0.5) 
         node [endomorphisms, anchor=south] (End0) {};
   \path (End0.north) ++ (0.0, 0) node [below, color=black] {$\text{End}(\mathcal{M})$}; 
   

   % Adding an endomorphism element 
   \path (End0.south) ++ (0.0, 0.3) node [dot] (e) {};      
   %\path (e) node [below] {$\rho_{0}(g)=\mathbf{S}_{0}$};    
   
   % Arrow going from x to Ex
   \path (e)+(-0.5,0.55) coordinate (c1);
   \path (e)+(0.5,0.55) coordinate (c2);   
   \path [draw, -stealth, line width=0.5,color=my_alejocol5a] (x) .. controls (c1) and (c2) .. (ex);   


   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%% Lie Algebra (original with Bracket product)%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   % Lie Algebra    
   \path (End0.north west) ++ (-4, 0) 
         node [algebra, anchor = north east, fill=my_alejocol2b!70] (At) {};   
   \path (At.north) ++ (0,-0.1) node [below,color=black] {$\mathfrak{g}$}; 
   \path (At.center) ++ (0,0) node [below,color=black] {$[X,Y]=Z$}; 
   \path (At.south) ++ (0,-0.1) node [below,color=black] {Lie Algebra};
   \path (At.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
   
   
   
%   % Subset in A_tilde  
%    \path (At.south) ++ (0,0.1) 
%    node [subendomor2in1, anchor=south,color=black!30] (subset2) {};
%    \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\tilde{\mathcal{C}}$};
    
    % Element in the Algebra
    %\path (At.south) ++ (0.0, 0.2) node [dot] (a2) {}; 
   
   
   
   
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Universal Enveloping Algebra U(g) %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (End0.north west) ++ (-1, 0) 
         node [algebra, anchor = north east] (A) {};   
   \path (A.north) ++ (0,-0.1) node [below,color=black] {$U(\mathfrak{g})$};
   \path (A.center) ++ (0,0) node [below,color=black] {$xy=z$};  
   \path (A.south) ++ (0,-0.1) node [below,color=black, align=center] {Universal\\ Enveloping \\Algebra};  
    
    
%    % Subset in the Algebra  
%    \path (A.south) ++ (0,0.1) 
%    node [subendomor2in1, anchor=south,color=black!30] (subset2) {};
%    \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\mathcal{C}$};
    
    % Element in the Algebra
    \path (A.south) ++ (0.0, 0.2) node [dot] (a1) {}; 
        
        
        
        
   % Arrow indicating \rho going from A to End(M)  
   \path (A.north) + (1,-0.6) coordinate (c1);
   \path (End0.north) + (-1,-0.6) coordinate (c2);   
   \path [draw, -stealth,line width = 1.0,color=green!60!black] (a1) .. controls (c1) and (c2) .. (e) node[midway,above left,rotate=0,color=green!60!black] {$\rho$};
   
   
   
   
   % Arrow going from Lie Algebra to universal Enveloping U(g)
   \path (A.south) + (-0.2,-0.5) coordinate (c2);
   \path (At.south) + (0.2,-0.5) coordinate (c1);   
   \path [->,draw, -stealth,line width = 1,color=black] (At.east) -- (A.west) node[midway,below,rotate=0,color=black] {$U$};




\end{tikzpicture}


}







==> source_figs/fig10/fig2_tikz_source.tex <==
%!TEX root = fig2_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%


%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{180, 222,44}
\definecolor{my_cp5_col3}{RGB}{94, 201, 98}
\definecolor{my_cp5_col4}{RGB}{33, 145, 140}
\definecolor{my_cp5_col5}{RGB}{59, 82, 139}
\definecolor{my_cp5_col6}{RGB}{68, 1, 84}


\usetikzlibrary{positioning,decorations.pathreplacing,shapes}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% SCALES AND BASIC QUANTITIES %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%--- Scale 
\def \scale {1.4}
\def \unit { \scale cm}

%%--- Vertical distance between blocks
\def \vertsep {1*\scale}

%%--- Horizontal distance between blocks
\def \horzsep {1*\scale}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%    SETTINGS OF BLOCKS USED IN THE PICTURE %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                    
% Block styles
 
\tikzstyle{myboxlabel} = [set,
fill=my_cp5_col3,
minimum width  = 1.61*\unit,
minimum height = 0.5*\unit]
 
 
                             

\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% BEGINNING OF PICTURE %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%-- Here I can choose the font size ----
{\fontsize{8}{8}\selectfont	
	
	
\begin{tikzpicture}[scale=\scale,rounded corners,ultra thick]



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Color Labels palette  %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


   %%------------ Label 1 --------
   
   \path (0,0) node [] (L1) {};
   \path (L1) ++ (0, 0) node [rotate=90, color=black] {Label 1};
   
   
   %%------------ Label 2 --------
   
    \path (L1.south)++(0,\vertsep) node [] (L2) {};
    \path (L2) ++ (0, 0) node [rotate=90, color=black] {Label 2};
    
    
     %%------------ Label 3 --------
     
     \path (L2.south)++(0,\vertsep) node [] (L3) {};
     \path (L3) ++ (0, 0) node [rotate=90, color=black] {Label 3};  
    
    
     %%------------ Label 4 --------
         
     \path (L3.south)++(0,\vertsep) node [] (L4) {};
     \path (L4) ++ (0, 0) node [rotate=90, color=black] {Label 4}; 
    
 

\end{tikzpicture}


}







==> source_figs/fig2/fig2_tikz_source.tex <==
%!TEX root = fig2_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%%-------Blue Colors of the Palette
\definecolor{my_alejocol5a}{RGB}{1,31,75}
\definecolor{my_alejocol4a}{RGB}{3,57,108}
\definecolor{my_alejocol3a}{RGB}{0,91,150}
\definecolor{my_alejocol2a}{RGB}{100,151,177}
\definecolor{my_alejocol1a}{RGB}{179,205,224}

%--------Red Colors of the Palette
\definecolor{my_alejocol4b}{RGB}{212, 220, 220}
\definecolor{my_alejocol3b}{RGB}{113, 18, 55}
\definecolor{my_alejocol2b}{RGB}{236, 85, 141}
\definecolor{my_alejocol1b}{RGB}{225, 73, 132}

%--------Blue-Green Colors of the Palette
\definecolor{my_alejocol4c}{RGB}{81, 185, 239}
\definecolor{my_alejocol3c}{RGB}{119, 164, 211}
\definecolor{my_alejocol2c}{RGB}{193, 223, 213}
\definecolor{my_alejocol1c}{RGB}{53, 89, 85}

%--Gray colors added to the pallette
\colorlet{my_alejocolg1}{black!30}
\colorlet{my_alejocolg2}{black!35}
\colorlet{my_alejocolg3}{black!40}
\colorlet{my_alejocolg4}{black!45}
\colorlet{my_alejocolg5}{black!50}
\colorlet{my_alejocolg6}{black!55}
\colorlet{my_alejocolg7}{black!60}



\usetikzlibrary{positioning,decorations.pathreplacing,shapes}
%\usepackage[english]{babel}
%\usepackage{microtype}
%\usepackage[hmargin=1.5cm,vmargin=1cm]{geometry}
%\usepackage{amsmath}
%\DeclareMathOperator{\p}{p}
%\newcommand*{\cancer}{\text{cancer}}
%\newcommand*{\testp}{\text{test}+}



%%%%%%%%%%%%%%%%%%%%%%%%%%% Settings of Blocks and picture %%%%%%%%%%%%%%%%%%%

\def \scale {1.3}
\def \unit  { \scale cm}
\def \layerinterdist {2.5}


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0.2*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                    
% Block styles
\tikzstyle{shadow_squared} = [rectangle,color=black,
rounded corners = 0.2*\unit,
fill=black,
inner sep=0pt,
draw,
anchor = south east,
line width=0.1mm,
minimum width  = 4.1*\unit,
minimum height = 3.9*\unit]                    
                    

                    
\tikzstyle{vectorspace} = [ set, 
                             fill=my_alejocol4c!50,
                             minimum width  = 1.5*\unit,
                             minimum height = 2.0*\unit]
                             
\tikzstyle{endomorphisms} = [ vectorspace,
                              fill=black!15,
                              minimum height = 1.3*\unit]
                                
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in1} = [endomorphisms, rounded corners=0.3*\unit,
                              fill=black!30,
                              minimum width  = 0.8*\unit,
                              minimum height = 0.8*\unit
                             ]                                                                                                                                                
\tikzstyle{algebra} = [ endomorphisms,
                        fill=my_alejocol2b!70,
                        minimum width = 1.5*\unit]

\tikzstyle{group_math} = [endomorphisms,
minimum width = 1.5*\unit,
minimum height = 0.5*\unit]


\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





{\fontsize{8}{8}\selectfont


\begin{tikzpicture}[rounded corners,ultra thick]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Shadow Under ASP Model %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 \path (0.9*\unit,-1.1*\unit) node [shadow_squared, opacity=0.2, fill=gray] (shadow1) {};
 %\path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};      






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Vector space M  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (0,0) node [vectorspace] (M0) {};
   \path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};
   
   % Element of the vector space
   \path (M0) ++ (-0.5,0.2) node [dot] (x) {};
   \path (x.south)++(0,-0.1) node [below, color=black] {$\mathbf{x}$}; 
   
   % Element filtered in the vector space
   \path (M0) ++ (0.5,0.2) node [dot] (ex) {};
   \path (ex.south) node [below, color=black] {$\rho(a)\mathbf{x}$};      
              

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Endomorphisms   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (M0.north) ++ (0, 0.5) 
         node [endomorphisms, anchor=south] (End0) {};
   \path (End0.north) ++ (0.0, 0) node [below, color=black] {$\text{End}(\mathcal{M})$}; 
   

   % Adding an endomorphism element 
   \path (End0.south) ++ (0.0, 0.3) node [dot] (e) {};      
   %\path (e) node [below] {$\rho_{0}(g)=\mathbf{S}_{0}$};    
   
   % Arrow going from x to Ex
   \path (e)+(-0.5,0.55) coordinate (c1);
   \path (e)+(0.5,0.55) coordinate (c2);   
   \path [draw, -stealth, line width=0.5,color=my_alejocol5a] (x) .. controls (c1) and (c2) .. (ex);   


   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%% Lie Algebra (original with Bracket product)%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   % Lie Algebra    
   \path (End0.north west) ++ (-4, 0) 
         node [algebra, anchor = north east, fill=my_alejocol2b!70] (At) {};   
   \path (At.north) ++ (0,-0.1) node [below,color=black] {$\mathfrak{g}$}; 
   \path (At.center) ++ (0,0) node [below,color=black] {$[X,Y]=Z$}; 
   \path (At.south) ++ (0,-0.1) node [below,color=black] {Lie Algebra};
   \path (At.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
   
   
   
   
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%% Lie Group %%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   % Lie Group   
   \path (At.south) ++ (0, -2.5) 
   node [group_math, anchor = center, fill=my_alejocolg1!50] (G) {};   
   \path (G.north) ++ (0,-0.1) node [below,color=black] {$G$}; 
   %\path (G.center) ++ (0,0) node [below,color=black] {$[X,Y]=Z$}; 
   \path (G.south) ++ (0,-0.1) node [below,color=black] {Lie Group};
   %\path (G.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
   
   
   

   
   
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Universal Enveloping Algebra U(g) %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (End0.north west) ++ (-1, 0) 
         node [algebra, anchor = north east] (A) {};   
   \path (A.north) ++ (0,-0.1) node [below,color=black] {$U(\mathfrak{g})$};
   \path (A.center) ++ (0,0) node [below,color=black] {$xy=z$};  
   \path (A.south) ++ (0,-0.1) node [below,color=black, align=center] {Universal\\ Enveloping \\Algebra};  
    
    
%    % Subset in the Algebra  
%    \path (A.south) ++ (0,0.1) 
%    node [subendomor2in1, anchor=south,color=black!30] (subset2) {};
%    \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\mathcal{C}$};
    
    % Element in the Algebra
    \path (A.south) ++ (0.0, 0.2) node [dot] (a1) {}; 
        
        
        
        
 
        
        
        
        
        
   % Arrow indicating \rho going from A to End(M)  
   \path (A.north) + (1,-0.6) coordinate (c1);
   \path (End0.north) + (-1,-0.6) coordinate (c2);   
   \path [draw, -stealth,line width = 1.0,color=green!60!black] (a1) .. controls (c1) and (c2) .. (e) node[midway,above left,rotate=0,color=green!60!black] {$\rho$};
   
   
   % Arrow going from Lie Algebra to universal Enveloping U(g)  
   \path [->,draw, -stealth,line width = 1,color=black] (At.east) -- (A.west) node[midway,below,rotate=0,color=black] {$U$};


    % Arrow going from Lie Algebra to Lie Group = Exponential Map  
    \path [->,draw, -stealth,line width = 1,color=black] (At.south)+(0,-1) -- (G.north) node[midway,right,rotate=0,color=black] {$e^{(\cdot)}$};



\end{tikzpicture}


}







==> source_figs/fig3/fig3_tikz_source.tex <==
%!TEX root = fig3_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%%-------Blue Colors of the Palette
\definecolor{my_alejocol5a}{RGB}{1,31,75}
\definecolor{my_alejocol4a}{RGB}{3,57,108}
\definecolor{my_alejocol3a}{RGB}{0,91,150}
\definecolor{my_alejocol2a}{RGB}{100,151,177}
\definecolor{my_alejocol1a}{RGB}{179,205,224}

%--------Red Colors of the Palette
\definecolor{my_alejocol4b}{RGB}{212, 220, 220}
\definecolor{my_alejocol3b}{RGB}{113, 18, 55}
\definecolor{my_alejocol2b}{RGB}{236, 85, 141}
\definecolor{my_alejocol1b}{RGB}{225, 73, 132}

%--------Blue-Green Colors of the Palette
\definecolor{my_alejocol4c}{RGB}{81, 185, 239}
\definecolor{my_alejocol3c}{RGB}{119, 164, 211}
\definecolor{my_alejocol2c}{RGB}{193, 223, 213}
\definecolor{my_alejocol1c}{RGB}{53, 89, 85}

%--Gray colors added to the pallette
\colorlet{my_alejocolg1}{black!30}
\colorlet{my_alejocolg2}{black!35}
\colorlet{my_alejocolg3}{black!40}
\colorlet{my_alejocolg4}{black!45}
\colorlet{my_alejocolg5}{black!50}
\colorlet{my_alejocolg6}{black!55}
\colorlet{my_alejocolg7}{black!60}



\usetikzlibrary{positioning,decorations.pathreplacing,shapes}
\usetikzlibrary{arrows}
%\usepackage[english]{babel}
%\usepackage{microtype}
%\usepackage[hmargin=1.5cm,vmargin=1cm]{geometry}
%\usepackage{amsmath}
%\DeclareMathOperator{\p}{p}
%\newcommand*{\cancer}{\text{cancer}}
%\newcommand*{\testp}{\text{test}+}



%%%%%%%%%%%%%%%%%%%%%%%%%%% Settings of Blocks and picture %%%%%%%%%%%%%%%%%%%

\def \scale {1.3}
\def \unit  { \scale cm}
\def \layerinterdist {2.5}


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0.2*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                    
% Block styles
\tikzstyle{shadow_squared} = [rectangle,color=black,
rounded corners = 0.2*\unit,
fill=black,
inner sep=0pt,
draw,
anchor = south east,
line width=0.1mm,
minimum width  = 4.1*\unit,
minimum height = 3.9*\unit]                    
                    

                    
\tikzstyle{vectorspace} = [ set, 
                             fill=my_alejocol4c!50,
                             minimum width  = 1.5*\unit,
                             minimum height = 2.0*\unit]
                             
\tikzstyle{endomorphisms} = [ vectorspace,
                              fill=black!15,
                              minimum height = 1.3*\unit]
                                
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in1} = [endomorphisms, rounded corners=0.3*\unit,
                              fill=black!30,
                              minimum width  = 0.8*\unit,
                              minimum height = 0.8*\unit
                             ]                                                                                                                                                
\tikzstyle{algebra} = [ endomorphisms,
                        fill=my_alejocol2b!70,
                        minimum width = 1.5*\unit]

\tikzstyle{group_math} = [endomorphisms,
minimum width = 1.5*\unit,
minimum height = 0.5*\unit]


\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





{\fontsize{8}{8}\selectfont


\begin{tikzpicture}[rounded corners,ultra thick]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Shadow Under ASP Model %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 \path (0.9*\unit,-1.1*\unit) node [shadow_squared, opacity=0.2, fill=gray] (shadow1) {};
 %\path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};      

 \path (-5.9*\unit,-1.1*\unit) node [shadow_squared, opacity=0.2, fill=gray] (shadow2) {};
 %\path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};    




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Vector space M  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (0,0) node [vectorspace] (M0) {};
   \path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};
   
   % Element of the vector space
   \path (M0) ++ (-0.5,0.2) node [dot] (x) {};
   \path (x.south)++(0,-0.1) node [below, color=black] {$\mathbf{x}$}; 
   
   % Element filtered in the vector space
   \path (M0) ++ (0.5,0.2) node [dot] (ex) {};
   \path (ex.south) node [below, color=black] {$\rho(a)\mathbf{x}$};      
              

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Endomorphisms   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (M0.north) ++ (0, 0.5) 
         node [endomorphisms, anchor=south] (End0) {};
   \path (End0.north) ++ (0.0, 0) node [below, color=black] {$\text{End}(\mathcal{M})$}; 
   

   % Adding an endomorphism element 
   \path (End0.south) ++ (0.0, 0.3) node [dot] (e) {};      
   %\path (e) node [below] {$\rho_{0}(g)=\mathbf{S}_{0}$};    
   
   % Arrow going from x to Ex
   \path (e)+(-0.5,0.55) coordinate (c1);
   \path (e)+(0.5,0.55) coordinate (c2);   
   \path [draw, -stealth, line width=0.5,color=my_alejocol5a] (x) .. controls (c1) and (c2) .. (ex);   








   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%% Lie Algebra (original with Bracket product)%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   % Lie Algebra    
   \path (End0.north west) ++ (-4, 0) 
         node [algebra, anchor = north east, fill=my_alejocol3a] (At) {};   
   \path (At.north) ++ (0,-0.1) node [below,color=black] {\textcolor{white}{$\mathfrak{g}$}}; 
   \path (At.center) ++ (0,0) node [below,color=black] {\textcolor{white}{$[X,Y]=Z$}}; 
   \path (At.south) ++ (0,-0.1) node [below,color=black] {Lie Algebra};
   \path (At.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
   
   
   
   
   
   
   
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%% L1(g) %%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   \path (At.north) ++ (0, 1) 
   node [algebra, anchor = south] (Lg) {};   
   \path (Lg.north) ++ (0,-0.1) node [below,color=black] {$L_1 (\mathfrak{g})$};
   \path (Lg.center) ++ (0,0) node [below,color=black] {$\tilde{f}: \mathfrak{g}\rightarrow\mathbb{C}$};  
   % \path (LUg.south) ++ (0,-0.1) node [below,color=black, align=center] {Universal\\ Enveloping \\Algebra};  
   
   
   %    % Subset in the Algebra  
   %    \path (A.south) ++ (0,0.1) 
   %    node [subendomor2in1, anchor=south,color=black!30] (subset2) {};
   %    \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\mathcal{C}$};
   
   % Element in the Algebra
  % \path (A.south) ++ (0.0, 0.2) node [dot] (a1) {}; 
   
   
   
   
   
   
   
   
   
   
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%  L1(G) - Group Algebra %%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    % Group Algebra
    \path (At.north west) ++ (-1, 0) 
    node [algebra, anchor = north east, fill=my_alejocol2b!70] (LG) {};   
    \path (LG.north) ++ (0,-0.1) node [below,color=black] {$L_1(G)$}; 
    \path (LG.center) ++ (0,0) node [below,color=black] {$f: G\rightarrow\mathbb{C}$}; 
    \path (LG.south) ++ (0,-0.1) node [below,color=black] {Group Algebra};
    %\path (LG.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
   
   
   
   
   
   
   
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%% Endomorphisms  for ASP model in L(G) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    \path (LG.west) ++ (-2, 0) 
    node [endomorphisms, anchor=center] (End1) {};
    \path (End1.north) ++ (0.0, 0) node [below, color=black] {$\text{End}(\mathcal{V})$}; 
    
    
    
    
    
    
    
    
    
    % Adding an endomorphism element 
    % \path (End1.south) ++ (0.0, 0.3) node [dot] (e1) {};      
    %\path (e) node [below] {$\rho_{0}(g)=\mathbf{S}_{0}$};    
    
%    % Arrow going from x to Ex
%    \path (e)+(-0.5,0.55) coordinate (c1);
%    \path (e)+(0.5,0.55) coordinate (c2);   
%    \path [draw, -stealth, line width=0.5,color=my_alejocol5a] (x) .. controls (c1) and (c2) .. (ex);   
    
   
   
   
   
   
   
   
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%% Vector space M for L(G) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   \path (End1.south)++(0,-0.5) node [vectorspace, anchor=north] (V) {};
   \path (V.south) ++ (0, 0) node [above, color=black] {$\mathcal{V}$};
   
%   % Element of the vector space
%   \path (V) ++ (-0.5,0.2) node [dot] (x) {};
%   \path (x.south)++(0,-0.1) node [below, color=black] {$\mathbf{x}$}; 
%   
%   % Element filtered in the vector space
%   \path (M0) ++ (0.5,0.2) node [dot] (ex) {};
%   \path (ex.south) node [below, color=black] {$\rho(a)\mathbf{x}$};      
%   
   
  
   
   
   
   
   
   
   
   
   
   
   
   
   
   
   
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%% Lie Group %%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   % Lie Group   
   \path (At.south) ++ (0, -2.5) 
   node [group_math, anchor = center, fill=my_alejocolg1!50] (G) {};   
   \path (G.north) ++ (0,-0.1) node [below,color=black] {$G$}; 
   %\path (G.center) ++ (0,0) node [below,color=black] {$[X,Y]=Z$}; 
   \path (G.south) ++ (0,-0.1) node [below,color=black] {Lie Group};
   %\path (G.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
   
   
   

   
   
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Universal Enveloping Algebra U(g) %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (End0.north west) ++ (-1, 0) 
         node [algebra, anchor = north east] (A) {};   
   \path (A.north) ++ (0,-0.1) node [below,color=black] {$U(\mathfrak{g})$};
   \path (A.center) ++ (0,0) node [below,color=black] {$xy=z$};  
   \path (A.south) ++ (0,-0.1) node [below,color=black, align=center] {Universal\\ Enveloping \\Algebra};  
    
    
%    % Subset in the Algebra  
%    \path (A.south) ++ (0,0.1) 
%    node [subendomor2in1, anchor=south,color=black!30] (subset2) {};
%    \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\mathcal{C}$};
    
    % Element in the Algebra
    \path (A.south) ++ (0.0, 0.2) node [dot] (a1) {}; 
        
        
        
        
 
 
 
 
 
 
 
 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%% ARROWS %%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
         
   % Arrow indicating \rho going from A to End(M)  
   \path (A.north) + (1,-0.6) coordinate (c1);
   \path (End0.north) + (-1,-0.6) coordinate (c2);   
   \path [draw, -stealth,line width = 1.0,color=green!60!black] (a1) .. controls (c1) and (c2) .. (e) node[midway,above left,rotate=0,color=green!60!black] {$\rho$};
   
 
   % Arrow going from Lie Algebra to universal Enveloping U(g)  
   \path [->,draw, -stealth,line width = 1,color=black] (At.east) -- (A.west) node[midway,below,rotate=0,color=black] {$U$};


    % Arrow going from Lie Algebra to Lie Group = Exponential Map  
    \path [->,draw, -stealth,line width = 1,color=black] (At.south)+(0,-1) -- (G.north) node[midway,right,rotate=0,color=black] {$e^{(\cdot)}$};

    
    % Arrow going from L(G) to L(g)
    \path [->,draw, -stealth,line width = 1,color=black,<->] (LG.north) -- (Lg.west) node[midway,left,rotate=0,color=black,align=center] {Kashiwara-Vergne Theorem\\ $f\ast_G h = \tilde{f} \ast_{L_1 (\mathfrak{g})} \tilde{h}$};


    % Arrow going from G to L(G)
    \path [draw, -stealth ,line width = 1,color=black,<->] (G.west) -- (LG.east) node[midway,left,rotate=0,color=black,align=center] {};


\end{tikzpicture}


}







==> source_figs/fig6/fig3_tikz_source.tex <==
%!TEX root = fig3_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%


%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{94, 201, 98}
\definecolor{my_cp5_col3}{RGB}{33, 145, 140}
\definecolor{my_cp5_col4}{RGB}{59, 82, 139}
\definecolor{my_cp5_col5}{RGB}{68, 1, 84}



\usetikzlibrary{positioning,decorations.pathreplacing,shapes}
\usetikzlibrary{arrows}




%%%%%%%%%%%%%%%%%%%%%%%%%%% Settings of Blocks and picture %%%%%%%%%%%%%%%%%%%




 


\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]




\tdplotsetmaincoords{0}{0} % view angles
\tdplotsetrotatedcoords{0}{0}{0} 



%% -- Number of elements in the grid
\def\gridnumber{6}
\def\imagesize{4}
\def\imagedotsize{5}


\def\scale{0.45}

{\fontsize{6}{6}\selectfont


\begin{tikzpicture}[scale=\scale, tdplot_rotated_coords, grid/.style={very thin,gray}]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% FIRST ROW IMAGES ON THE GRID %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%-----------------------------------------------
%%------------ ORIGINAL REGUALR GRID ---------------
%%-----------------------------------------------

%draw a grid in the x-y plane
\foreach \x in {0,1,...,\gridnumber}
\foreach \y in {0,1,...,\gridnumber}
{
	\draw[grid,rotate=0,my_cp5_col3,line width=1*\scale] (\x,0) -- (\x,\gridnumber);
	\draw[grid,rotate=0,my_cp5_col3,line width=1*\scale] (0,\y) -- (\gridnumber,\y);
};


% Drawing the pixels that indicate the image
\foreach \x in {1,...,\imagesize}
\foreach \y in {1,...,\imagesize}
{
\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
}



%%-----------------------------------------------
%%----------- IMAGE ON REGUALR GRID ---------------
%%-----------------------------------------------

% Drawing the pixels that indicate the image
\begin{scope}[shift={(\gridnumber+1.6,-0.5)},rotate=10]
\foreach \x in {1,...,\imagesize}
\foreach \y in {1,...,\imagesize}
{
	\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
}
\end{scope}


% Drawing the pixels that indicate the image
\begin{scope}[shift={(\gridnumber+1,0)},rotate=0]
\foreach \x in {0,1,...,\gridnumber}
\foreach \y in {0,1,...,\gridnumber}
{
	\draw[grid,rotate=0,my_cp5_col3,line width=1*\scale] (\x,0) -- (\x,\gridnumber);
	\draw[grid,rotate=0,my_cp5_col3,line width=1*\scale] (0,\y) -- (\gridnumber,\y);
};
\end{scope}




%%-----------------------------------------------
%%------------ IMAGE ON REGUALR GRID --------------
%%-----------------------------------------------

% Drawing the pixels that indicate the image

\begin{scope}[shift={(2*\gridnumber+2,0)},rotate=0]
\foreach \x in {0,1,...,\gridnumber}
\foreach \y in {0,1,...,\gridnumber}
{
	\draw[grid,rotate=0,my_cp5_col3,line width=1*\scale] (\x,0) -- (\x,\gridnumber);
	\draw[grid,rotate=0,my_cp5_col3,line width=1*\scale] (0,\y) -- (\gridnumber,\y);
};
\end{scope}


% Drawing the pixels that indicate the image
\begin{scope}[shift={(2*\gridnumber+2,0)},rotate=0]
\foreach \x in {1,...,\imagesize}
\foreach \y in {1,...,\imagesize}
{
	\draw[fill=my_cp5_col3, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
};
\end{scope}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% SECOND ROW HOW TO DO INTERPOLATION  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%---------------------------------------------------
%%----------- IMAGE ON REGUALR DOT-GRID --------------
%%---------------------------------------------------


% Drawing the pixels that indicate the image
\begin{scope}[shift={(0,-\gridnumber-1)},rotate=0]
\foreach \x in {0,1,...,\imagedotsize}
\foreach \y in {0,1,...,\imagedotsize}
{
	%\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
	%\node[circle,draw=black,fill=white!80!black,minimum size=20] () at (\x+0.5,\y+0.5) {d};
	\pgfmathtruncatemacro{\label}{\x + 5 * (4 - \y)+6};
	\node[dot,draw=black,fill=white,minimum size=15*\scale, opacity=0.5]
	(\label) at (\x+0.5,\y+0.5) {\label};
}
\end{scope}


% Drawing the pixels that indicate the image
\begin{scope}[shift={(0,-\gridnumber-1)},rotate=0]
\foreach \x in {1,...,\imagesize}
\foreach \y in {1,...,\imagesize}
{
	%\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
	%\node[circle,draw=black,fill=white!80!black,minimum size=20] () at (\x+0.5,\y+0.5) {d};
	\pgfmathtruncatemacro{\label}{\x + 5 * (4 - \y)+6};
	\node[dot,draw=black,fill=my_cp5_col2,minimum size=15*\scale, opacity=0.7]
	(\label) at (\x+0.5,\y+0.5) {\label};
}
\end{scope}



%%----------------------------------------------
%%----------- IMAGE ON REGUALR GRID --------------
%%----------------------------------------------

% Drawing the pixels that indicate the image
\begin{scope}[shift={(\gridnumber+1,-\gridnumber-1)},rotate=0]
\foreach \x in {0,1,...,\imagedotsize}
\foreach \y in {0,1,...,\imagedotsize}
{
	%\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
	%\node[circle,draw=black,fill=white!80!black,minimum size=20] () at (\x+0.5,\y+0.5) {d};
	\pgfmathtruncatemacro{\label}{\x + 5 * (4 - \y)+6};
	\node[dot,draw=black,fill=white,minimum size=15, opacity=0.5]
	(u\label) at (\x+0.5,\y+0.5) {\label};
}
\end{scope}


% Drawing the pixels that indicate the image
\begin{scope}[shift={(\gridnumber+1.6,-\gridnumber-1-0.5)},rotate=10]
\foreach \x in {1,...,\imagesize}
\foreach \y in {1,...,\imagesize}
{
	%\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
	%\node[circle,draw=black,fill=white!80!black,minimum size=20] () at (\x+0.5,\y+0.5) {d};
	\pgfmathtruncatemacro{\label}{\x + 5 * (4 - \y)+6};
	\node[dot,draw=black,fill=my_cp5_col2,minimum size=15, opacity=0.7]
	(v\label) at (\x+0.5,\y+0.5) {\label};
}
\end{scope}


%%---------- Neightborhood for interpolation ------------------

\node[circle,fill=my_cp5_col4,draw,opacity=0.4,inner sep=20pt] () at (u7){};


\node[dot,draw=black,fill=my_cp5_col3,minimum size=15, opacity=0.7](u7) at (u7) {7};


%%----------------------------------------------
%%----------- IMAGE ON REGUALR GRID --------------
%%----------------------------------------------

% Drawing the pixels that indicate the image
\begin{scope}[shift={(2*\gridnumber+2,-\gridnumber-1)},rotate=0]
\foreach \x in {0,1,...,\imagedotsize}
\foreach \y in {0,1,...,\imagedotsize}
{
	%\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
	%\node[circle,draw=black,fill=white!80!black,minimum size=20] () at (\x+0.5,\y+0.5) {d};
	\pgfmathtruncatemacro{\label}{\x + 5 * (4 - \y)+6};
	\node[dot,draw=black,fill=white,minimum size=15, opacity=0.5]
	() at (\x+0.5,\y+0.5) {\label};
}
\end{scope}


% Drawing the pixels that indicate the image
\begin{scope}[shift={(2*\gridnumber+2,-\gridnumber-1)},rotate=0]
\foreach \x in {1,...,\imagesize}
\foreach \y in {1,...,\imagesize}
{
	%\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
	%\node[circle,draw=black,fill=white!80!black,minimum size=20] () at (\x+0.5,\y+0.5) {d};
	\pgfmathtruncatemacro{\label}{\x + 5 * (4 - \y)+6};
	\node[dot,draw=black,fill=my_cp5_col3,minimum size=15, opacity=0.7]
	() at (\x+0.5,\y+0.5) {\label};
}
\end{scope}





%% Drawing the pixels that indicate the image
%\begin{scope}[shift={(\gridnumber+1.6,-0.5)},rotate=10]
%
%
%\foreach \x in {1,...,\imagesize}
%\foreach \y in {1,...,\imagesize}
%{
%	\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
%}
%
%\end{scope}
%
%
%% Drawing the pixels that indicate the image
%\begin{scope}[shift={(\gridnumber+1,0)},rotate=0]
%
%\foreach \x in {0,1,...,\gridnumber}
%\foreach \y in {0,1,...,\gridnumber}
%{
%	\draw[grid,rotate=0,my_cp5_col3,line width=1] (\x,0) -- (\x,\gridnumber);
%	\draw[grid,rotate=0,my_cp5_col3,line width=1] (0,\y) -- (\gridnumber,\y);
%};
%
%\end{scope}



\end{tikzpicture}   


}







==> source_figs/fig7/fig2_tikz_source.tex <==
%!TEX root = fig2_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%-- Four colors Color Palette
\definecolor{my_cp4_col1}{RGB}{255, 86, 87}
\definecolor{my_cp4_col2}{RGB}{55, 108, 138}
\definecolor{my_cp4_col3}{RGB}{242, 217, 187}
\definecolor{my_cp4_col4}{RGB}{99, 143, 169}

%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{94, 201, 98}
\definecolor{my_cp5_col3}{RGB}{33, 145, 140}
\definecolor{my_cp5_col4}{RGB}{59, 82, 139}
\definecolor{my_cp5_col5}{RGB}{68, 1, 84}





\usetikzlibrary{positioning,decorations.pathreplacing,shapes}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% SCALES AND BASIC QUANTITIES %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%--- Scale 
\def \scale {1.4}
\def \unit { \scale cm}

%%--- Vertical distance between blocks
\def \vertsep {0.5*\scale}

%%--- Horizontal distance between blocks
\def \horzsep {0.5*\scale}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%    SETTINGS OF BLOCKS USED IN THE PICTURE %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0.2*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                    
% Block styles
\tikzstyle{shadow_squared} = [rectangle,color=black,
rounded corners = 0.2*\unit,
fill=black,
inner sep=0pt,
draw,
anchor = south east,
line width=0.1mm,
minimum width  = 4.1*\unit,
minimum height = 3.9*\unit]                    
                    

                    
\tikzstyle{vectorspace} = [ set, 
                             fill=my_cp5_col4,
                             minimum width  = 1.61*\unit,
                             minimum height = 1*\unit]
 
                             
\tikzstyle{endomorphisms} = [ vectorspace,
                              fill=my_cp5_col3,
                              minimum width  = 1.61*\unit,
                              minimum height = 1*\unit]
                                
                                
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in1} = [endomorphisms, rounded corners=0.2*\unit,
                              fill=black!30,
                              minimum width  = 1.2*\unit,
                              minimum height = 0.5*\unit
                             ]    
                             
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in2} = [endomorphisms, rounded corners=0.2*\unit,
fill=black!30,
minimum width  = 0.5*\unit,
minimum height = 0.5*\unit
]                                
 
                                                                                                                                                                         
\tikzstyle{algebra} = [ endomorphisms,
                        fill=my_cp5_col2]


\tikzstyle{group_math} = [endomorphisms]



\tikzstyle{liea_bracket} = [endomorphisms]



\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% BEGINNING OF PICTURE %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%-- Here I can choose the font size ----
{\fontsize{8}{8}\selectfont	
	
	
\begin{tikzpicture}[scale=\scale,rounded corners,ultra thick]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Shadow Under ASP Model %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 %\path (0.9*\unit,-1.1*\unit) node [shadow_squared, opacity=0.2, fill=gray] (shadow1) {};
 %\path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};      






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Vector space M  %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (0,0) node [vectorspace,fill=my_cp5_col5] (M0) {};
   \path (M0.south) ++ (0, 0) node [below, color=black] {$\mathcal{H}$};
   
   % Element of the vector space
   \path (M0) ++ (-0.5,0.2) node [dot,color=white] (x) {};
   \path (x.south)++(0,-0.1) node [below, color=white] {$\mathbf{x}$}; 
   
   % Element filtered in the vector space
   \path (M0) ++ (0.5,0.2) node [dot,color=white] (ex) {};
   \path (ex.south) node [below, color=white] {$\widehat{p_{\epsilon}(\mathcal{S})}\mathbf{x}$};      
     
              



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Endomorphisms   %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (M0.north) ++ (0, \vertsep) node [endomorphisms, anchor=south,fill=my_cp5_col4] (End0) {};
   \path (End0.north) ++ (0.0, 0) node [above, color=black] {$\mathcal{B}(\mathcal{H})$}; 

  %%----------------------
  %%---- Image of approximated Group Algebra
  
  \path (End0.south) ++ (0, 0.1) 
  node [ subendomor2in1, anchor = south, fill=my_cp5_col4!50] (Endhat) {};  
  \path (Endhat.north) ++ (0,-0.05) node [above,color=white] {$\rho( L^{1}(\widehat{G}))$};    

  %%----------------------
  %%---- Adding elements inside the boxes

   % Adding an endomorphism element 
   \path (End0.center) ++ (-0.5, 0.2) node [dot] (e) {};      
   \path (e) node [above,color=white] {$\rho(\boldsymbol{a})$};    
   
   % Adding an endomorphism element 
   \path (Endhat.south) ++ (0.0, 0.1) node [dot] (eepsilon) {};      
   \path (eepsilon) node [above] {$\widehat{p_{\epsilon}(\mathcal{S})}$};  
   
   % Arrow going from x to Ex
   \path (eepsilon)+(-0.5,0.4) coordinate (c1);
   \path (eepsilon)+(0.5,0.4) coordinate (c2);   
   \path [draw, -stealth, line width=0.5,color=my_cp5_col3] (x) .. controls (c1) and (c2) .. (ex);   

  

  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Algebra %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (End0.north west) ++ (-\horzsep, 0) 
         node [algebra, anchor = north east,fill=my_cp5_col3] (A) {};   
   \path (A.north) ++ (0,0.0) node [above,color=black] {$\mathcal{A} = L^{1}(G)$};
   %\path (A.center) ++ (0,0) node [below,color=black] {$xy=z$};  
   % \path (A.south) ++ (0,-0.1) node [below,color=black, align=center] {Lie Group \\ Algebra};  

  %%----------------------
  %%---- Approximated Group Algebra
  %%----------------------  
  
  \path (A.south) ++ (0, 0.1) 
  node [ subendomor2in1, anchor = south, fill=my_cp5_col3!50] (LGhat) {};    
  \path (LGhat.north) ++ (0,-0.05) node [above,color=black] {$ L^{1}(\widehat{G})$};  
    
    % Element in the Algebra
    \path (LGhat.south) ++ (0.0, 0.1) node [dot] (pepsilon) {}; 
   \path (pepsilon.north) ++ (0,0.0) node [above,color=black] {$p_{\epsilon}(\widehat{\mathcal{G}})$};    
        
    % Element in the Algebra L1(G)
    \path (A.center) ++ (0.5, 0.2) node [dot] (a1) {}; 
    \path (a1.north) ++ (0,0.0) node [above,color=black] {$\boldsymbol{a}$};   
   
   
   
        
   
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%% Lie Group %%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
  % Lie Group   
  \path (A.north west) ++ (-\horzsep, 0) 
  node [group_math, anchor = north east, fill=my_cp5_col2] (G) {};   
  \path (G.north) ++ (0,0) node [above,color=black] {$G$}; 
  %\path (G.center) ++ (0,0) node [below,color=black] {$[X,Y]=Z$}; 
 % \path (G.south) ++ (0,-0.1) node [below,color=black] {Lie Group};
  %\path (G.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
    
 %%----------------------
 %%---- Approximated Group from discretization of t in exp(tX) 
 %%----------------------  
 
 \path (G.south) ++ (0, 0.1) 
  node [ subendomor2in1, anchor = south, fill=my_cp5_col2!50] (Ghat) {}; 
  \path (Ghat.north) ++ (0,0.0) node [above,color=black] {$\widehat{G}$};  

  %%----------------------
  %%---- Subset of generators in the approximated Lie Group
  %%----------------------  
  
  \path (Ghat.center) ++ (0, 0) 
  node [ subendomor2in2, anchor = center, fill=my_cp5_col2!30] (Ghatgen) {}; 
  \path (Ghatgen) ++ (0,0.0) node [color=black] {$\widehat{\mathcal{G}}$};     
        
 
 
 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%% Lie Algebra Bracket  %%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
  % Lie Algebra Bracket  
  \path (G.south) ++ (0, -\vertsep) 
  node [liea_bracket, anchor = north, fill=my_cp5_col1] (gbracket) {};   
  \path (gbracket.south) ++ (0,0) node [below,color=black] {$(\mathfrak{g},[\cdot,\cdot])$}; 
  %\path (G.center) ++ (0,0) node [below,color=black] {$[X,Y]=Z$}; 
 % \path (G.south) ++ (0,-0.1) node [below,color=black] {Lie Group};
  %\path (G.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
     
  %%----------------------
  %%---- Subset of generators in the LieBracket Algebra
  %%----------------------  
  
  \path (gbracket.center) ++ (0, 0) 
  node [ subendomor2in2, anchor = center, fill=my_cp5_col1!50] (gbracketgen) {}; 
  \path (gbracketgen) ++ (0,0.0) node [color=black] {$\mathfrak{G}$};  
 
 
 
 
 
 
        
        
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%% ARROWS %%%%%%%%%%%%%%%%%%%%%%      
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      
  

%    % Arrow going from Lie Algebra to Lie Group = Exponential Map 
%    \path (A.west) ++ (0.15, 0) node [] (a1) {};  
%    \path [->,draw, -stealth,line width = 0.5,color=black] (G.east) -- (a1) node[midway,right,rotate=0,color=black] {};

  
     % Arrow indicating \rho going from A to End(M)  
     \path (A.north) + (1,0) coordinate (c1);
     \path (End0.north) + (-1,0) coordinate (c2);   
     \path [draw, -stealth,line width = 0.5,color=black] (a1) .. controls (c1) and (c2) .. (e)  node[midway,above ,rotate=0,color=black] {$\rho$};
        
        
   % Arrow indicating \rho going from A to End(M)  
   \path (A.north) + (1,-0.5) coordinate (c1);
   \path (End0.north) + (-1,-0.5) coordinate (c2);   
   \path [draw, -stealth,line width = 0.5,color=black] (pepsilon) .. controls (c1) and (c2) .. (eepsilon) node[midway,below left,rotate=0,color=black] {$\hat{\rho}$};
   

    % Arrow going from Lie Group to Lie Group Algebra
   %\path (A.south) ++ (0.0, -0.6) node [] (a1) {};  
   \path [->,draw, -stealth,line width = 0.5,color=black] (G.east) -- (A.west) node[midway,right,rotate=0,color=black] {};


    % Exponential Map grom the Lie bracket algebra into the Lie group G
    \path [->,draw, -stealth,line width = 0.5,color=black] (gbracket.north) -- (G.south) node[midway,right,rotate=0,color=black] {$e^{\mathfrak{g}t}$};


     % Exponential Map grom the Lie bracket algebra into the Lie group G
     \node (a) at (gbracket.center) {};
     \node (b) at (Ghat.center) {};
     \path [->, draw, -stealth,line width = 0.5,color=black] (a) edge [bend left]  node[midway,left,rotate=0,color=black] {$e^{\mathfrak{G}n\epsilon}$} (b);


\end{tikzpicture}


}







==> source_figs/fig8/fig2_tikz_source.tex <==
%!TEX root = fig2_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%-- Four colors Color Palette
\definecolor{my_cp4_col1}{RGB}{255, 86, 87}
\definecolor{my_cp4_col2}{RGB}{55, 108, 138}
\definecolor{my_cp4_col3}{RGB}{242, 217, 187}
\definecolor{my_cp4_col4}{RGB}{99, 143, 169}

%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{94, 201, 98}
\definecolor{my_cp5_col3}{RGB}{33, 145, 140}
\definecolor{my_cp5_col4}{RGB}{59, 82, 139}
\definecolor{my_cp5_col5}{RGB}{68, 1, 84}





\usetikzlibrary{positioning,decorations.pathreplacing,shapes}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% SCALES AND BASIC QUANTITIES %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%--- Scale 
\def \scale {1.4}
\def \unit { \scale cm}

%%--- Vertical distance between blocks
\def \vertsep {0.5*\scale}

%%--- Horizontal distance between blocks
\def \horzsep {0.5*\scale}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%    SETTINGS OF BLOCKS USED IN THE PICTURE %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0.2*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                    
% Block styles
\tikzstyle{shadow_squared} = [rectangle,color=black,
rounded corners = 0.2*\unit,
fill=black,
inner sep=0pt,
draw,
anchor = south east,
line width=0.1mm,
minimum width  = 4.1*\unit,
minimum height = 3.9*\unit]                    
                    

                    
\tikzstyle{vectorspace} = [ set, 
                             fill=my_cp5_col4,
                             minimum width  = 1.61*\unit,
                             minimum height = 1*\unit]
 
                             
\tikzstyle{endomorphisms} = [ vectorspace,
                              fill=my_cp5_col3,
                              minimum width  = 1.61*\unit,
                              minimum height = 1*\unit]
                                
                                
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in1} = [endomorphisms, rounded corners=0.2*\unit,
                              fill=black!30,
                              minimum width  = 1.2*\unit,
                              minimum height = 0.5*\unit
                             ]    
                             
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in2} = [endomorphisms, rounded corners=0.2*\unit,
fill=black!30,
minimum width  = 0.5*\unit,
minimum height = 0.5*\unit
]                                
 
                                                                                                                                                                         
\tikzstyle{algebra} = [ endomorphisms,
                        fill=my_cp5_col2]


\tikzstyle{group_math} = [endomorphisms]



\tikzstyle{liea_bracket} = [endomorphisms]



\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% BEGINNING OF PICTURE %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%-- Here I can choose the font size ----
{\fontsize{7}{7}\selectfont	
	
	

\begin{tikzpicture}[every tree node/.style={},
level distance=1.25cm,sibling distance=1mm, 
edge from parent path={(\tikzparentnode) -- (\tikzchildnode)}]



\Tree [.\node[fill=my_cp5_col2] {$\mathbf{I}$}; 
%%
%%------ Descending from S1 ------
%%
[.\node[fill=my_cp5_col3] {$\mathbf{S}_1$};  
%\edge node[auto=right] {Help!};  
              [.\node[fill=my_cp5_col4,text=my_cp5_col1]{$\mathbf{S}_{1}^{2}$}; {$\cdots$} {$\cdots$} {$\cdots$}  ] 
              [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_1 \mathbf{S}_2 $}; {$\cdots$} {$\cdots$} {$\cdots$}   ] 
              [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_1 \mathbf{S}_3 $}; {$\cdots$} {$\cdots$} {$\cdots$}   ] 
]
%%
%%------ Descending from S2 ------
%%
[.\node[fill=my_cp5_col3] {$\mathbf{S}_2$}; 
              [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_{2} \mathbf{S}_1$}; {$\cdots$} {$\cdots$} {$\cdots$}  ] 
              [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_{2}^2$}; {$\cdots$} {$\cdots$} {$\cdots$}  ] 
              [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_{2}\mathbf{S}_{3}$}; {$\cdots$} {$\cdots$} {$\cdots$}  ] 
] 
%%
%%------ Descending from S3 ------
%%
[.\node[fill=my_cp5_col3] {$\mathbf{S}_3$}; 
             [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_{3} \mathbf{S}_1$}; {$\cdots$} {$\cdots$} {$\cdots$}  ] 
             [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_{3}\mathbf{S}_{2}$};  {$\cdots$} {$\cdots$} {$\cdots$}  ] 
             [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_{3}^2$}; {$\cdots$} {$\cdots$} {$\cdots$}  ] 
] 
]
\end{tikzpicture}
}







==> source_figs/fig9/fig2_tikz_source.tex <==
%!TEX root = fig2_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%


%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{180, 222,44}
\definecolor{my_cp5_col3}{RGB}{94, 201, 98}
\definecolor{my_cp5_col4}{RGB}{33, 145, 140}
\definecolor{my_cp5_col5}{RGB}{59, 82, 139}
\definecolor{my_cp5_col6}{RGB}{68, 1, 84}


\usetikzlibrary{positioning,decorations.pathreplacing,shapes}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% SCALES AND BASIC QUANTITIES %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%--- Scale 
\def \scale {1.4}
\def \unit { \scale cm}

%%--- Vertical distance between blocks
\def \vertsep {0.5*\scale}

%%--- Horizontal distance between blocks
\def \horzsep {1*\scale}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%    SETTINGS OF BLOCKS USED IN THE PICTURE %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                    
% Block styles
 
\tikzstyle{myboxlabel} = [set,
fill=my_cp5_col3,
minimum width  = 1.61*\unit,
minimum height = 0.5*\unit]
 
 
                             

\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% BEGINNING OF PICTURE %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%-- Here I can choose the font size ----
{\fontsize{8}{8}\selectfont	
	
	
\begin{tikzpicture}[scale=\scale,rounded corners,ultra thick]



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Color Labels palette  %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


   %%------------ Label 1 --------
   
   \path (0,0) node [myboxlabel,fill=my_cp5_col1] (L1) {};
   \path (L1.south) ++ (0, 0) node [below, color=black] {Label 1};
   
   
   %%------------ Label 2 --------
   
    \path (L1.east)++(\horzsep,0) node [myboxlabel,fill=my_cp5_col2] (L2) {};
    \path (L2.south) ++ (0, 0) node [below, color=black] {Label 1};
    
    
     %%------------ Label 3 --------
     
     \path (L2.east)++(\horzsep,0) node [myboxlabel,fill=my_cp5_col3] (L3) {};
     \path (L3.south) ++ (0, 0) node [below, color=black] {Label 1};  
    
    
     %%------------ Label 4 --------
         
     \path (L3.east)++(\horzsep,0) node [myboxlabel,fill=my_cp5_col4] (L4) {};
     \path (L4.south) ++ (0, 0) node [below, color=black] {Label 1}; 
    
 
      %%------------ Label 5 --------
      
      \path (L4.east)++(\horzsep,0) node [myboxlabel,fill=my_cp5_col5] (L5) {};
      \path (L5.south) ++ (0, 0) node [below, color=black] {Label 1};    
    

      %%------------ Label 6 --------
      
      \path (L5.east)++(\horzsep,0) node [myboxlabel,fill=my_cp5_col6] (L6) {};
      \path (L6.south) ++ (0, 0) node [below, color=black] {Label 1};      
    
    
    
%   % Element of the vector space
%   \path (M0) ++ (-0.5,0.2) node [dot,color=white] (x) {};
%   \path (x.south)++(0,-0.1) node [below, color=white] {$\mathbf{x}$}; 
%   
%   % Element filtered in the vector space
%   \path (M0) ++ (0.5,0.2) node [dot,color=white] (ex) {};
%   \path (ex.south) node [below, color=white] {$\widehat{p_{\epsilon}(\mathcal{S})}\mathbf{x}$};      
%     



\end{tikzpicture}


}






